CkIO: Parallel File Input for Over-Decomposed Task-Based Systems

Parallel input performance issues are often neglected in large scale parallel applications in Computational Science and Engineering. Traditionally, there has been less focus on input performance because either input sizes are small (as in biomolecular simulations) or the time doing input is insignificant compared with the simulation with many timesteps. But newer applications, such as graph algorithms add a premium to file input performance. Additionally, over-decomposed systems, such as Charm++/AMPI, present new challenges in this context in comparison to MPI applications. In the over-decomposition model, naive parallel I/O in which every task makes its own I/O request is impractical. Furthermore, load balancing supported by models such as Charm++/AMPI precludes assumption of data contiguity on individual nodes. We develop a new I/O abstraction to address these issues by separating the decomposition of consumers of input data from that of file-reader tasks that interact with the file system. This enables applications to scale the number of consumers of data without impacting I/O behavior or performance. These ideas are implemented in a new input library, CkIO, that is built on Charm++, which is a well-known task-based and overdecomposed-partitions system. CkIO is configurable via multiple parameters (such as the number of file readers and/or their placement) that can be tuned depending on characteristics of the application, such as file size and number of application objects. Additionally, CkIO input allows for capabilities such as effective overlap of input and application-level computation, as well as load balancing and migration. We describe the relevant challenges in understanding file system behavior and architecture, the design alternatives being explored, and preliminary performance data.

==> IEEEstyling/texstyling.tex <==
\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.


==> bibliography.tex <==
\section*{Acknowledgment}
% \section*{References}

% Please number citations consecutively within brackets \cite{b1}. The 
% sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
% number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
% the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

% Number footnotes separately in superscripts. Place the actual footnote at 
% the bottom of the column in which it was cited. Do not put footnotes in the 
% abstract or reference list. Use letters for table footnotes.

% Unless there are six authors or more give all authors' names; do not use 
% ``et al.''. Papers that have not been published, even if they have been 
% submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
% that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
% Capitalize only the first word in a paper title, except for proper nouns and 
% element symbols.

% For papers published in translation journals, please give the English 
% citation first, followed by the original foreign-language citation \cite{b6}. 

%\begin{thebibliography}{00}
% \bibitem{b1} P. Jetley, F. Gioachin, C. Mendes, L. V. Kale, and T. R. Quinn. Massively parallel cosmological simulations with ChaNGa. In Proceedings of IEEE International Parallel and Distributed Processing Symposium 2008, 2008.



%\end{thebibliography}

==> design.tex <==
\section{Design and Implementation} \label{Design and Implementation}
When implementing CkIO's input infrastructure in the Charm++ framework and API, we decided to augment the existing CkIO output infrastructure in order to both have synergy in design between input and output, but also to make it familiar to users of the CkIO output API if they want to integrate CkIO input into their own program. 
\subsection{Director Chare}
The director chare is responsible for coordinating the actions of the PEs early on in the CkIO input process. When a read session is declared, the director broadcasts a message, indicating that a new session has started, to the Manager group, which will be discussed in more detail later.

\subsection{Manager Group}
The \textit{manager} is a group that is shared with CkIO's output. It is responsible for maintaining a table, mapping each read session to a ReadAssembler group. Additionally, the manager is responsible for assigning the tags for the zero-copy data transfer used when transferring the data from buffer chares to the clients.

\subsection{ReadAssembler Group}
The \textit{ReadAssembler} is a group that is responsible for fulfilling the read requests made to the CkIO input library. The ReadAssembler will tag incoming read requests for a session, request the necessary data from the Buffer Chares that have the data of a read request, and then assemble the read together and return it to the user via the user-specified callback.

\subsection{Buffer Chares}
Within CkIO Input, \textit{buffer chares} are the key component of the architecture. Buffer chares are the chares that interact directly with the file system and read the file into memory, later to be served over the network. Each buffer chare reads a disjoint section of the file. The number of buffer chares is selected manually by the programmer. This is what allows the programmer to optimize the input performance of their application without changing the number of clients. A visual representation of how buffer chares fit into the input model is shown in Figure \ref{fig:bufferChares}


\subsection{Callback-centric API}
The base CkIO input API heavily utilizes callbacks in order to allow the Charm++ runtime system to have enough freedom to schedule work optimally. We will briefly give an overview about the base CkIO input API, and will show a more complete example program in Section 5.

\begin{itemize}
    \item \textit{Ck::IO::open(...)} - responsible for opening the file and informing the other PEs about it
    \item \textit{Ck::IO::startReadSession(...)} - used to prefetch a section of a seekable file into memory by making the buffer chares read. The input is asynchronous, allowing for it to be overlapped with computation, as described later.
    \item \textit{Ck::IO::read(...)} - This is the function by which application chares will read, giving CkIO an offset and number of bytes with respect to the overall file. When the read is complete, will invoke a user-specified callback with the result.
    \item \textit{Ck::IO::closeReadSession(...)} - This allows the user to clean up the buffer chares. Frees the memory used to store the session data.
    \item \textit{CK::IO::close(...)} - Closes the file across all of the PEs. 
\end{itemize}

\subsection{Supporting concurrent background work}

In order to allow for input to be efficiently overlapped with other application computation, we make sure to do non-blocking reads. For each buffer chare, we spawn a new OS-level thread whose sole responsibility is to read the section of the read session its buffer chare is responsible for. This will allow the application to continue while the I/O from the buffer chare is being completed. If a read requests occurs before the I/O is completed, that read request will simply be buffered until the I/O is finished; afterwards, the read request will be fulfilled. We also note that, since the spawned thread is only doing I/O, it will hinder the performance of the application code. 
    

==> figures-tex/fixed-bg.tex <==
\begin{figure}

  \centering
  
 \includegraphics[width=0.8\linewidth]{figures/fixed-bg.pdf}
   \caption{Runtime comparison between CkIO input and naive Charm-based input, with fixed background work. Results collected on a single node of Bridges2, using up to 64 cores. Both approaches read a 4GB file and launched a Charm group to compute a fixed amount of background work (darker shade) concurrently. Each data point denotes the minimum time recorded over 5 runs, to avoid capturing unnecessary variability. The lighter bar plus its corresponding darker bar together make up the total runtime, to demonstrate proportion of background work.}
   \label{fig:fixed-bg}

\end{figure}

==> figures-tex/naive-input-performance.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/naive-baseline-bridges.png}
  \caption{Naive Input on Bridges2}
  \label{fig:bridgesnaive}
\end{subfigure}%

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/naive-baseline-frontier.png}
  \caption{Naive Input on Frontier}
  \label{fig:frontiernaive}
\end{subfigure}
\caption{Naive over-decomposed input on Bridges and Frontier, using 16 nodes and 512 PEs on both machines for each run. Each data point denotes an average runtime over 10 sample runs reading from a single variable-sized file. The x-axis marks the number of clients, or the over-decomposition factor used for the read.}
\label{fig:naiveinput}
\end{figure*}
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/naive-baseline-bridges.png}
%     \caption{Naive over-decomposed input on Bridges, using 16 RM nodes and 512 PEs on both machines for each run. Each data point denotes an average runtime over 10 sample runs reading from a single variable-sized file. The x-axis marks the number of clients, or the over-decomposition factor used for the read.}
% \end{figure*}

==> optimizations.tex <==
\section{Optimizations}
We support the following optimizations regarding file input: \begin{itemize}
    \item Selective reads prefetch only the necessary data. To support this, we require that the user specifies what portion of the file they would like to read from. 
    \item The number of input-designated chares is chosen independently of the number of application chares (clients) that need data. This allows us to chose the best decomposition for input regardless of the users constraints.
    \item We support concurrent background work, allowing applications to stay active while I/O completes, effectively overlapping the I/O time with useful computations.
    \item The ability for the application to migrate tasks across processors in order to attain better input performance in their application. 
\end{itemize}

%Buffer chares read in the data of the session greedily. While this can take a lot of memory for the buffer chares to store this data, it can allow for speed ups in some applications (what applications??). 

\subsection{Selective pre-fetching}
In order to accomplish our first objective of pre-fetching and reading only the necessary data, we introduce the concept of a \textit{read session}. The read session is a component of the CkIO API which must be initialized before any reading begins. On initialization, a read session requires which requires the name, start byte, and end byte of a single file that the user will query. Given this initial information, CkIO can begin to greedily read in the input data for the section of the file that is relevant to the application. This greedy reading of data is one component that allows for the overlapping of the I/O with other application level computation and messaging, which will be described in more detail. In addition, when large files that cannot fit into memory directly, this allows the user to essentially read in the file that can fit into memory chunk-by-chunk, which works around any memory constraints of the system.

Additionally, because the selective pre-fetching maintains the data in memory, this I/O schema is amenable to forms of parallelism, such as pipeline parallelism. To show this at a high level, imagine a program in which every worker is required to perform some computation on elements of a file in a block-cyclic fashion. That is, if there are $n$ workers, the $i^{th}$ worker will be assigned the ${j^{th}}$ element if $j \equiv i \mod n$. Also assume that a worker must complete the work of one element before consuming their next element. Because the reads in our scheme are non-blocking and can be scheduled by the runtime, the worker can issue the read request for the next element before executing the work for their current element. This allows for the read to commence while the worker is doing its computation, effectively overlapping communication and computation. 

\subsection{Independent decomposition of file input vs application}

The basic idea behind CkIO, which helps it accomplish its goals of supporting overdecomposition and migratability, is the separation of file input decomposition from application decomposition via a two-phase input implementation. Our library aims to support application developers with performant file input regardless of how they chose to over-decompose their application. To do this, CkIO uses an intermediary chare array designated for input, called the \textit{buffer chare} array, which sits between the file system and the application chares, or \textit{clients}. Figure~\ref{fig:diagram} shows how the layer of buffer chares abstracts the interaction with the file system from the application.

\input{figures-tex/bc-diagram}

The buffer chares are responsible for reading disjoint sections of a file that an application will need. The number of buffer chares should be configured by the application to decompose the file-system interaction optimally, depending on a number of factors including the number of PEs, number of nodes, and amount of data to be read. When a client requests data via the CkIO infrastructure, this request is forwarded to and handled by the buffer chare responsible for the relevant data.

By introducing this intermediary layer that sits between the clients and the file system, the actual input performance of reading the data from the file system can be optimized regardless of the client decomposition. This two-phase structure incurs the slight overhead of additional interconnect data transfer from buffer chare to client, but because the interconnects on most supercomputing clusters are much faster than the I/O disks, the improved input time much outweighs any network cost. Figure~\ref{fig:naivevsckio} shows how CkIO provides consistent performance regardless of application decomposition.

\input{figures-tex/naiveVSckio}

\subsection{Overlapping input with concurrent computation}
The CkIO library is built to allow any concurrent computation from the application to overlap input, hiding file system latency. CkIO achieves this by spawning an OS-level thread for each buffer chare performing a read. This thread is then responsible for performing the I/O for the data that its corresponding buffer chare is responsible for.

Mini benchmark showing overlap for the two different implementations.

